A hybrid approach for semantic enrichment of MathML mathematical expressions

In this paper, we present a new approach to the semantic enrichment of mathematical expression problem. Our approach is a combination of statistical machine translation and disambiguation which makes use of surrounding text of the mathematical expressions. We first use Support Vector Machine classifier to disambiguate mathematical terms using both their presentation form and surrounding text. We then use the disambiguation result to enhance the semantic enrichment of a statistical-machine-translation-based system. Experimental results show that our system archives improvements over prior systems.

==> respodn.tex <==
We would like to express our sincere appreciation to all the reviewers for providing the valuable comments.
Following are the detailed response to the comments.

Reviewer 1 comments:

1. "the category of the mathematical expression" is mentioned several times (e.g. p. 2) without any explanation.
- The category of the mathematical expression is the name of the category in the Wolfram Function Site that a mathematical expression belongs to. Examples include "Bessel Functions", "Hankel Functions", ... We will add more details about the category of the mathematical expression in section 3.2 (page 5).
2. The shorthand SMT should be defined.
- We will add a discussion about SMT method, and its shorthand in section 2 (page 3).

Reviewer 2 comments:

1. To my knowledge Snuggletex is geared towards a particular physics domain, thus it is not surprising that interpretations of constants are always the same. This should be mentioned.
- We will check this fact and mention this in section 2 (page 2-3).
2. Most major CAS (Maple and Mathematica at least) have a translator for presentation to content MathML. Obviously, these translation depend very much on the underlying interpretation in the respective CAS of the input syntax. Nevertheless, it would be fair to mention this as related work.
- Yes, these work related to our study. We will mention this in section 2 (page 3).
3. You only seem to consider "font-free" expressions. However, mathematical meaning can often vary, when the fonts vary. (Good example, is Planck's constant, that is even a specialist Unicode symbol in v1.0). How would the SVM be able to deal with font specs in the math tags?
- In this paper, we use the name of the identifier as a feature. If two identifiers have different Unicode symbol (different name), then the SVM can distinguish them. We, however, did not consider the style of the font (italic, bold), since we do not have the data that contains this information. The font style is a good feature so we will consider it in future work.
4. It will be interesting to see how the approach scales. Maybe by the time of the CRC you can elaborate on the last sentence in the conclusion a bit.
- We will take into account your comments and make change in section 5 (page 9).

Reviewer 3 comments:

1. Maybe the authors should discuss more the distinction between "mathematical named entities" (i.e., constants, functions, formulas which have names) and ordinary variables/functions, etc., because it looks like their system works best for the former.
- We will take into account your comments and make change in section 1 (page 1).
2. Also it would be interesting to compare whether usage of a specific notation in the ACL corpus is correlated with bibliographic references (in other words, whether notation is inherited from previous papers).
- The correlation between notation and bibliographic reference is an interesting information. We will consider about it in future work.

Reviewer 4 comments:

1. GIZA++ should be introduced with more detail. The citation supposed to reference GIZA points to a general overview paper that mentions giza only once in its own references. As the alignment is a central part of the method, it merits more detail.
- We will add more details about GIZA in the paper, and cite to more detail paper.
2. The content mathml elements with fixed meaning, such as "Golden Ratio" should be csymbol elements, not ci. ci elements denote a variable.
- In our collected data (the expressions from Wolfram Functions Site), "Golden Ratio" is marked as "ci". We also think the correct element is "csymbol". We will substitute this with another example.
3. The disambiguation is limited in targeting cases of lexical ambiguity, assuming no structural ambiguity exists (e.g. which operation is performed first in "sin x/y").
- In the scope of this paper, we only disambiguate lexical ambiguities. Structural ambiguities should also be consider to achieve better results. We will mention it in the future work.
4. The examples in table 3 are structurally very basic. Providing additional examples of alignment and translation of non-trivially aligning presentation and content trees is strongly encouraged.
- We will select and add more examples from ACL-ARC data to table 3.
